Actor-Based Model Checking for SDN Networks

Software-Defined Networking (SDN) is a networking paradigm that has become increasingly popular in the last decade. The unprecedented control over the global behavior of the network it provides opens a range of new opportunities for formal methods and much work has appeared in the last few years on providing bridges between SDN and verification. This article advances this research line and provides a link between SDN and traditional work on formal methods for verification of concurrent and distributed software---actor-based modelling. We show how SDN programs can be seamlessly modelled using \emph{actors}, and thus existing advanced model checking techniques developed for actors can be directly applied to verify a range of properties of SDN networks, including consistency of flow tables, violation of safety policies, and forwarding loops. Our model checker for SDN networks is available through an online web interface, that also provides the SDN actor-models for a number of well-known SDN benchmarks.

==> actors.tex <==
% ;; -*- coding: iso-latin-1; TeX-PDF-mode: t; TeX-master: "main" -*-%
%
%\newcommand{\ifle}[0]{\key{if}}
%
%\secbeg
%\subsection{The Actor Language}
%\secbeg
%
%We consider a simple actor language with three instructions which
%characterize the asynchronous execution model: (1) \textsf{new} $C$
%creates a new actor (with its own processor and queue of pending
%tasks) that executes tasks running methods of class $C$ and can only
%access its own memory, (2) \textsf{Fut f=a!m($\overline{x}$)} spawns
%an asynchronous task \textsf{m($\overline{x}$)} that is added to the
%queue of pending tasks of \textsf{a}, where \textsf{f} is a future
%variable that will allow us to check if such task has been completed,
%and (3) the instruction \textsf{await f?}  used to synchronize with
%the termination of the task associated to \textsf{f}, by releasing the
%processor (so that another task can be scheduled) if the task is not
%finished. It can be used also with boolean conditions \textsf{await
%  b?}  to suspend the execution of the current active task until
%condition \textsf{b} holds.  Tasks from different actors execute in
%parallel and task selection is \emph{non-deterministic}.  The grammar
%below describes the syntax of our programs:
%
%
%%\medskip
%
%\(
%\begin{array}{lll}
%  M & {:}{:}{=} & T~m(\bar{T}~\bar{x})\{s;\}\\
%  s & {:}{:}{=}  & s~;~s \mid x=e \mid 
%  \ifle~\mathit{b}~\iftethen~s~\ifteelse~s  \mid
%                   \while~\mathit{b}~\whilebody~\mathit{s} \mid  x.m({\bar{z}}) \\
%  &&  \mid  x=\newb~C(\bar{y})   \mid f=x!m({\bar{z}})
%     \mid \await{f}~ \mid \await{b}\\
%\end{array} 
%\)
%
%%\medskip
%
%
%
%\noindent
%where $x$, $y$, $z$ denote variables names, $f$ a future variable
%name, and $s$ a sequence of instructions.  For any entity $A$, the
%notation $\bar{A}$ is used as a shorthand for $A_1,...,A_n$.  We use
%the special actor identifier \texttt{this} to denote the current
%actor.  For the sake of generality, the syntax of expressions $e$,
%boolean conditions $b$ and types $T$ is not specified. As in the
%object-oriented paradigm, a class denotes a type of actors including
%their behavior, and it is defined as a set of fields and methods.  The
%``$.$'' in method calls, such as in $x.m({\bar{z}})$, denotes standard
%(synchronous) method calls, while ``$!$'' is used for asynchrony.  The
%formal semantics of the language is included in Appendix \ref{sec:semant-actor-lang}.
%
%We now illustrate it via an example.
%  The
% language is kept simple to explain the contributions of the paper in a
% clear way.




==> background_pkt.tex <==
% ;; -*- coding: iso-latin-1; TeX-PDF-mode: t; TeX-master: "main" -*-%


\newcommand{\ifle}[0]{\key{if}}


\section{Semantics for SDN Networks and for Actors}\label{sec:semant-sdn-netw}


\subsection{SDN Networks}\label{sec:sdn-networks} \fxnote{UCM: write this section}

\mz{Elvira, please write a couple of sentences here to introduce the
  section}

\begin{figure}[t]
\centering	
\includegraphics[scale=.27]{SDNInfoFlowDiag}
\caption{Information flow in SDN networks} 
\label{fig:sdn-infoflow}
\end{figure}

Figure~\ref{fig:sdn-infoflow} shows the information flow of packets
and messages among the different elements in a SDN network. As in
standard networks, packets can be sent from hosts to switches and
viceversa, and also from switches to switches (see dashed arrows). The
leftmost dashed arrow represents the reception by a host of a new
packet which is feed into the network.  The specific communications of
SDN networks are performed by means of \emph{Openflow messages} (see
regular arrows), which in our simplification can be of three
types\mz{MIght include here and in the diagram barrier messages and
  say they will be explained later}:

\begin{itemize}
\item \textsf{Packet-in}: This message is sent from a switch to the
  controller when the switch processes a packet for which it has no
  action rule to apply. The message includes the switch identifier and
  the identifier and header of the packet. The packet is buffered in
  the switch until a message of type \emph{Packet-out} is received.
\item \textsf{Modify-State}: This message is sent from the controller
  to a switch with new action rules to be inserted into the switch's
  flow-table. The message includes a flow-table entry with an action
  rule.
\item\textsf{Packet-out}: This message is sent from the controller to
  a switch to notify it must re-try applying an action rule to a
  buffered packet. The message includes the packet header.
\end{itemize}


Figure~\ref{sdn_semantics} show the semantics of the flow of
communications performed in our simplified SDN networks. 
%
The three types of messages below are respectively abbreviated as
\textsf{pktIn}, \textsf{modState} and \textsf{pktOut}. A host is a
term of the form $h(id,sid,in)$, where $id$ is the host identifier,
$sid$ the switch identifier to which the host is connected, and $in$
its input communications channel. A switch is of the form
$s(id,ft,b,in)$, where $id$ is the switch identifier, $ft$ its
flow-table, $b$ its internal buffer of packets and $in$ its input
channel. The controller is of the form $c(top,in)$ where $top$ is the
topology of the network and $in$ is its input channel.
%
A state of the SDN network is a tuple of the form
$\langle H,S,C \rangle$ where $H = \{h ~|~ h \text{ is a host}\}$,
$S = \{s ~|~ s \text{ is a switch}\}$, that is, $H$ is a set of hosts,
$S$ is a set of switches, and, $C$ is the controller.
%
Letter $p$ denotes a packet. Function $dest(p)$ returns the identifier
of the destination host or switch of packet $p$, and $header(p)$
returns its header.
%
Flow-tables are represented as mappings from packet headers to actions
and are treated as a black-box through the following functions:
$lookup(ft,ph)$ that returns the action associated to the packet with
header $ph$ in the flow-table $ft$, or $\bot$ if there is no entry for
it; and, $insert(ft,ph \mapsto a)$ that returns the new flow-table
after inserting in $ft$ the entry $ph \mapsto a$. For simplicity, we
only consider actions of the form $send(id)$, which indicates that the
corresponding packet should be sent to the host or switch with $id$ as
identifier.
%
% Actions are of the form $send(id)$. Hence a flow-table entry of the
% form $ph \mapsto send(id)$ indicates that the packet with header $ph$
% should be sent to the host or switch with $id$ as identifier. The
% notation $ft[ph \mapsto a]$ stands for storing/accesing entry
% $ph \mapsto a$ on flow-table $ft$, whereas $ft[ph \cancel{\mapsto}\_]$
% indicates that $ft$ does not contain an entry for $ph$.
%
Function $applyPol(top,sid,ph)$ represents the application of the
controllers's policy using the current network topology $top$ in
result to a packet with header $ph$ that the switch with identifier
$sid$ has not been able to handle. It returns a set of pairs
$\langle id,m\rangle$ where $m$ is a $id$ is the switch identifier
\mz{I am rewriting this} \textsf{modifyState} messages with associated
new flow-table entries to be forwarded to the corresponding switches.

A \emph{transition} or \emph{step} in the network corresponds to the
processing of a packet or message by a host, switch or the
controller. There are six (sets of) transition rules corresponding to
the different types of incoming arrows in
Figure~\ref{fig:sdn-infoflow}:

\begin{itemize}
\item \textsf{sendIn} (abbreviated as \textsc{si}): It corresponds to
  the processing by a host of a new packet which is feed into the
  network, in which case the packet is forwarded to the switch to
  which the host is connected.
%
\item \textsf{hostHandlePacket} (\textsc{hhp}): This corresponds to
  the processing by a host $h$ of a packet whose destination is $h$,
  in which case the packet is consumed without any further action.
%
\item \textsf{switchHandlePacket} (\textsc{shp}): When a switch
  processes a received packet, either from a host or from another
  switch, there are three cases: (cases 1 and 2) there is a send
  action rule in the switch's flow-table, hence the packet is
  forwarded to the host (case 1) or switch (case 2) indicated in the
  action; or (case 3) there is no rule for this packet, in which case
  the packet is buffered and a \textsf{Packet-in} message is sent to
  the controller.
%
\item \textsf{controlHandleMessage} (\textsc{chm}): The controller
  receives a \textsf{Packet-in} message from a switch $s$ in result to
  a packet that the switch $s$ has not been able to handle. As a
  result, the controller sends a set of \textsf{Modify-State} messages
  with new action rules to a selected set of switches (as specified by
  the controller's policy with the current network topology), and a
  \textsf{Packet-out} message to switch $s$.
%
\item \textsf{switchHandleMessage} (\textsc{shm}): It corresponds to
  the processing of a \textsf{Modify-State} message by a switch, in
  which case the received action rule is inserted into the switch's
  flow-table.
%
\item \textsf{sendOut} (\textsc{so}): This corresponds to the
  processing of a \textsf{Packet-out} message by a switch. There are
  three cases which are analogous to those of
  \textsf{switchHandlePacket} except that the packet is in the
  switch's buffer (instead of in its input channel), and that if no
  action rule is found in the switch's flow-table the packet is
  dropped.
\end{itemize}


\newcommand{\rrrule}[2]{
\begin{array}{c}
#1 \\
\hline\\[-0.25cm] 
#2 
\end{array}
\vspace*{0.0cm}
}

\begin{figure}[t]

{\small\begin{center}
 \textsc{(si)}~$\rrrule
 {h = h(id,sid,in \cup \{pkt\}),~~s = s(sid,ft,b,in'),~~ dest(pkt) \neq id}
 {\langle \{h\} \cup H, \{s\} \cup S, C\rangle \rightarrow
   \langle \{h(id,sid,in)\} \cup H, \{s(sid,ft,b,in' \cup \{pkt\})\} \cup S, C\rangle}
 $
\end{center}}

{\small\begin{center}
 \textsc{(hhp)}~$\rrrule
 {h = h(id,sid,in \cup \{pkt\}),~~ dest(pkt) = id}
 {\langle \{h\} \cup H, S, C\rangle \rightarrow
   \langle \{h(id,sid,in)\} \cup H, S, C\rangle}
 $
\end{center}}

{\small\begin{center}
 \textsc{(shp$_1$)}~$\rrrule
 {s = s(sid,ft,b,in \cup \{pkt\}),~~h = h(id,sid,in'),
   ~~ send(id) = lookup(ft,header(pkt))}
 {\langle \{h\} \cup H, \{s\} \cup S, C\rangle \rightarrow
   \langle \{h(id,sid,in' \cup \{pkt\})\} \cup H, \{s(sid,ft,b,in)\} \cup S, C\rangle}
 $
\end{center}}

{\small\begin{center}
 \textsc{(shp$_2$)}~$\rrrule
 {s = s(sid,ft,b,in \cup \{pkt\}),~~ s' = s(sid',ft',b',in'),
   ~~ send(id') = lookup(ft,header(pkt))}
 {\langle H, \{s,s'\} \cup S, C\rangle \rightarrow
   \langle H, \{s(sid,ft,b,in), s(sid',ft',b',in' \cup \{pkt\})\} \cup S, C\rangle}
 $
\end{center}}

{\small\begin{center}
 \textsc{(shp$_3$)}~$\rrrule
 {s{=}s(sid,ft,b,in \cup \{pkt\}),~ s' = s(sid,ft,b',in),~ \bot = lookup(ft,header(pkt)),~
  b'{=}b \cup \{pkt\}}
 {\langle H, \{s\} \cup S, c(top,in')\rangle \rightarrow
   \langle H, \{s'\} \cup S, c(top,in' \cup \{\mathsf{pktIn(sid,id(pkt),header(pkt))}\})\rangle}
 $
\end{center}}

{\small\begin{center}
 \textsc{(so$_1$)}~$\rrrule
 {s = s(sid,ft,b \cup \{pkt\},in \cup \{\mathsf{pktOut(ph)}\}),\\ ph=header(pkt),~~h = h(id,sid,in'),~~
  send(id) = lookup(ft,header(pkt))}
 {\langle \{h\} \cup H, \{s\} \cup S, C\rangle \rightarrow
   \langle \{h(id,sid,in' \cup \{pkt\})\} \cup H, \{s(sid,ft,b,in)\} \cup S, C\rangle}
 $
\end{center}}

{\small\begin{center}
 \textsc{(so$_2$)}~$\rrrule
 {s = s(sid,ft,b \cup \{pkt\},in \cup \{\mathsf{pktOut(ph)}\}),\\ ph=header(pkt),~~ s' = s(sid',ft',b',in'),~~
  send(sid') = lookup(ft,header(pkt))}
 {\langle H, \{s,s'\} \cup S, C\rangle \rightarrow
   \langle H, \{s(sid,ft,b,in), s(sid',ft',b',in' \cup \{pkt\})\} \cup S, C\rangle}
 $
\end{center}}

{\small\begin{center}
 \textsc{(so$_3$)}~$\rrrule
 {s = s(sid,ft,b \cup \{pkt\},in \cup \{\mathsf{pktOut(ph)}\}), ph=header(pkt),~~
  \bot = lookup(ft,header(pkt))}
 {\langle H, \{s\} \cup S, C\rangle \rightarrow
   \langle H, \{s(sid,ft,b,in)\} \cup S, C\rangle}
 $
\end{center}}

{\small\begin{center}
 \textsc{(shm)}~$\rrrule
 {s = s(sid,ft,b,in \cup \{\mathsf{modState(ph \mapsto a)}\})}
 {\langle H, \{s\} \cup S, C\rangle \rightarrow
   \langle H, \{s(sid,insert(ft,ph \mapsto a),b,in)\} \cup S, C\rangle}
 $
\end{center}}


{\small\begin{center}
 \textsc{(chm)}~$\rrrule
 {c = c(top,cin \cup \{\mathsf{pktIn(sid,pid,ph)}\}),~~
  s = s(sid,ft,b,sin),\\ ms = applyPol(top,sid,ph),~~
  ms_{id} = \{m ~|~ \langle id,m\rangle \in ms \},~~\\ 
  S' = \{s(sid',ft',b',in')~|~ s(sid',ft',b',in) \in S,
  in' = in \cup ms_{sid'}\} %sid' \neq sid, 
  }
 {\langle H, S \cup \{s\}, c\rangle \rightarrow
   \langle H, S' \cup s(sid,ft,b,sin \cup ms_{sid} \cup \{\mathsf{pktOut(ph)}\}), c(top,cin)\rangle}
 $
\end{center}}

\caption{Semantics of SDN networks}\label{sdn_semantics}
\end{figure}



\subsection{Syntax and Semantics for Actor Programs}\label{semantics}
\fxnote{UCM: revise/extend this section}

The grammar below describes the syntax of the actor programs in which
SDN models will be defined:


\medskip

\(
\begin{array}{lll}
 M & {:}{:}{=} & T~m(\bar{T}~\bar{x})\{s;\}\\
 s & {:}{:}{=}  & s~;~s \mid x=e \mid 
 \ifle~\mathit{b}~\iftethen~s~\ifteelse~s  \mid
                  \while~\mathit{b}~\whilebody~\mathit{s} \mid  x.m({\bar{z}}) \\
 &&  \mid  x=\newb~C(\bar{y})   \mid f=x!m({\bar{z}})
    \mid \await{f}~ \mid \await{b}\\
\end{array} 
\)

\medskip



\noindent
where $x$, $y$, $z$ denote variables names, $f$ a future variable
name, and $s$ a sequence of instructions.  For any entity $A$, the
notation $\bar{A}$ is used as a shorthand for $A_1,...,A_n$.  We use
the special actor identifier \texttt{this} to denote the current
actor.  For the sake of generality, the syntax of expressions $e$,
boolean conditions $b$ and types $T$ is left unspecified. As in the
object-oriented paradigm, a class denotes a type of actors including
their behavior, and it is defined as a set of fields and methods.  The
``$.$'' in method calls, such as in $x.m({\bar{z}})$, denotes standard
(synchronous) method calls, while ``$!$'' is used for asynchrony. 



\begin{figure}[t]
{\begin{center}


{\begin{center}
$\rrrule{
  \buffer(\objid,\bot,\heap,\queue)=\selectObject(\state), 
  \task(\tkid,m,\tv,s) = \selectTask(\buffer(\objid,\bot,\heap,\queue)), s  \not = \epsilon,   \state  \microstepstar{\objid\cdot \tkid} \state'   
 }
 {\textsc{(mstep)}~~~~~~~~~~~~~~~~~~~~~~~~~~~~ \hspace{2cm} \state
   \macrostep{} %{\objid\cdot   \tkid} 
\state' ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~} $
\end{center}\medskip\medskip

}

\medskip

$\rrrule{\taskId=\task(\tkid,m,l, \futvar{x}=y~!~m_1(\many{z});s),
  \objid_1=\tv(y),\tkid_1=\text{fresh}(),l_1{=}{\it newlocals}(\bar{z},m_1,l)}
 { \textsc{(asy)}~~~~~~~~~~~~~~~~~~~~~~~~~~~~ \buffer(\objid,\tkid, \heap,\queue \cup \{\taskId\})\sepo
 \buffer(\objid_1,\tkid',\heap', \queue')\rrderiv~~~~~~~~~~~~~~~~~~~~~~~~~ \\ 
\buffer(\objid,\tkid, \heap,  \queue {\cup} \{\task(\tkid,m,l[\futvar{x}{\mapsto}t_1],s)\})\sepo \buffer(\objid_1,\tkid',\heap',  \queue' {\cup} \{\task(\tkid_1,m_1,\tv_1,\body{m_1})\})}$
\end{center}
}
\medskip
{\begin{center}
$\rrrule{~~~~~~~\taskId=\task(\tkid,m,l,{x=\key{new}~D(\bar{y});s}),\objid_1{=}\text{fresh}(),\\
  {\textsc{(new)}}~~~~~~~~~~h'=\newheap(D),l'=l[x\rightarrow
  \objid_1], \key{class}~D(\bar{f})\{\ldots\}~~~~~~~~~~~~~~~~~~~~~~~}
 {\buffer(\objid,\tkid,h, \queue  \cup  \{\taskId \} )
\rrderiv 
{\buffer(\objid,\tkid,h, \queue  \cup \{\task(\tkid,m,l',s)\}) \sepo
  \buffer(\objid_1,\bot,h'[\bar{f} \mapsto \tv(\bar{y})],\emptyset)}}$
\end{center}
}
\medskip

  {\begin{center}
  \textsc{(await)$_1$}~$\rrrule{\taskId = \task(\tkid,m,\tv,\key{await}~\futvar{x};s),   
     \tv(\futvar{x})=\tkid_1,~ \task(\tkid_1,m_1,\tv_1, \epsilon) \in \state}
  {\buffer(\objid,\tkid, \heap, \queue \cup \{\taskId\}) 
  \rrderiv   \buffer(\objid,\tkid, \heap,\queue \cup \{\task(\tkid,m,\tv,s)\})} $
  \end{center}
  }
\medskip
  {\begin{center}
 \textsc{(await)$_2$}~$\rrrule{\taskId=\task(\tkid,m,\tv,\key{await}~\futvar{x};s),
    \tv(\futvar{x})=\tkid_1,~ \task(\tkid_1,m_1,\tv_1,\epsilon) \not \in \state}
  {\buffer(\objid,\tkid, \heap, \queue \cup \{\taskId\}) 
  \rrderiv  \buffer(\objid,\bot,\heap,  \queue \cup \{\task(\tkid,m,\tv,\key{await}~\futvar{x};s)\}) } $
  \end{center}
  }
\medskip
{\begin{center}
 \textsc{(return)}~$\rrrule{\taskId =\task(\tkid,m,\tv,\epsilon)}
 {\buffer(\objid,\tkid,\heap,\queue \cup \{\taskId\}) 
 \rrderiv  
 \buffer(\objid,\bot,\heap, \queue\cup \{\taskId\})}$
 \end{center}
 }
\secbeg
 \caption{Semantics of concurrent primitives of actor programs}\label{Summarized_semantics_await}
\secbeg\secbeg
\end{figure}

Figure~\ref{Summarized_semantics_await} presents the semantics of the
actor model. An \emph{actor} is a term
$\buffer(\objid,\tkid,\heap,\queue)$, where $\objid$ is the actor
identifier, $\tkid$ is the identifier of the \emph{active task} that
holds the actor's lock or $\bot$ if the actor's lock is free, $\heap$
is its local heap and $\queue$ is the set of tasks in the actor. A
{\em heap} $\heap$ is a mapping
$\heap :\Fields(C) \mapsto \mathbb{V}$, 
where 
$\mathbb{V}$
stands for the set of references and values.
%=\mathbb{Z} \cup \Refe \cup \{\key{null}\}$ and $\Refe$
%stands for the set of references of the form $\objid$. 
A \emph{task}
$\taskId$ is a term $\task(\tkid,m,l,s)$ where $\tkid$ is a unique
task identifier, $m$ is the method name executing in the task, $\tv$
is a mapping from local variables to $\mathbb{V}$, and $s$ is the
sequence of instructions to be executed.
%
As actors do not share their states, the semantics can be
presented as a macro-step semantics \cite{DBLP:conf/fase/SenA06}
(defined by means of the transition ``$\macrostep{}$'') in which the
evaluation of all statements of a task takes place serially (without
interleaving with any other task) until it gets to a \emph{release
  point}, i.e., a point in which the actor's processor becomes idle
due to the return or an await instruction. In this case, rule {\sc (mstep)} is
applied to select an available task from an actor, namely function
$\selectObject(\state)$ is applied to select \emph{non-deterministically} an actor
$\buffer(\objid,\bot,h,\queue)$ in the state with a non-empty queue $\queue$, and,
$\selectTask(\buffer(\objid,\bot,h,\queue))$ to select \emph{non-deterministically} a task of
$\queue$. % Macro-step transitions are usually labeled as
% $\macrostep{\objid\cdot\tkid}$, being $\objid \cdot \tkid$ the actor
% identifier $\objid$ and task identifier $\tkid$ selected (in rule {\sc (mstep)}).
% The actor identifier is sometimes omitted from the label if it is not
% relevant.
Micro-step transitions are written $\rrderiv$ and define
evaluations within a given macro-step.
%
As before, the sequential
instructions are standard and thus omitted.  In {\sc (new)}, an active
task $\taskId$ in actor  $\objid$ creates a new actor of class
$D$ with a fresh identifier $\objid_1=\text{fresh}()$, which is
introduced to the state with a free lock. Here $h'=\newheap(D)$ stands
for a default initialization on the fields of class $D$.  Rule {\sc
  (asy)} spawns a new task (the initial state is created by $\it
newlocals$) with a fresh task identifier $\tkid_1$ which is
stored in the future variable $\futvar{x}$.  We assume $\objid
\neq \objid_1$, but the case $\objid = \objid_1$ is analogous, the new
task  $\tkid_1$ is simply added to the queue $\queue'$ of
actor $\objid_1$.
In rule {\sc (await)$_1$},
the future variable $\futvar{x}$ we are awaiting for points to a
finished task and thus the \key{await} can be completed. The finished
task identified with $\tkid_1$ is looked up in all actors in the
current state (written as $\task(\tkid_1,m_1,\tv_1, \epsilon) \in
\state$).  Otherwise, {\sc (await)$_2$} yields the lock so that any
other task of the same actor can take it. The behaviour of {\sc await}
on boolean conditions is analogous. 
When rule {\sc (return)} is executed, the task is \emph{finished},
but it remains in the queue so that rules {\sc
  (await)$_1$} and {\sc (await)$_2$} can be applied.
%
A derivation $\ex \equiv
\state_0 \macrostep{} \cdots \macrostep{} \state_n$ is {\em complete}
if $\state_0$ is the initial state and all actors in $\state_n$ are of
the form $\buffer(\objid,\bot,\heap,\queue)$, where for all $\taskId
\in \queue$ it holds that $\taskId \equiv
\task(\tkid,m,\tv,\epsilon)$.


==> sdn.tex <==
% ;; -*- coding: iso-latin-1; TeX-PDF-mode: t; TeX-master: "main" -*-%


\section{Background: SDN Networks and Actors}



\subsection{SDN Networks}




\subsection{Syntax and Semantics for Actor Programs}


==> table.tex <==
% ;; -*- coding: iso-latin-1; TeX-PDF-mode: t; TeX-master: "main" -*-%


\begin{table}[t] \scriptsize
\centering \setlength{\tabcolsep}{.5mm}
 \begin{tabular}{|l|c|c|c|c|}\hline
% & \multicolumn{5}{c}{\textbf{DPOR}} \\%&
                                     %  \multicolumn{4}{c}{\textbf{entry-indep}}  & \multicolumn{3}{c}{\textbf{Reduction gains}}\\ 
%\cmidrule(l{0em}){2-5} %\cmidrule(l){4-5}\cmidrule(l){6-7}\cmidrule(l){8-10}\cmidrule(l){11-13}
   \textbf{Name} &  \textbf{Switch x Host x Packet} &  \textbf{Execs}  & \textbf{States}  & \textbf{Time}   \\ \hline
%& \textbf{Time} & \textbf{Execs} & \textbf{Time} & \textbf{Execs} & \textbf{Time} & \textbf{Execs} & \textbf{Time} & \textbf{~M} & \textbf{G%1} & \textbf{G2} & \textbf{G3}  \\ \toprule
%\cmidrule(l{0em}){1-10} 
 LB &  3x3x1/3x4x2  &   8/92 & 64/761 & 15/263   \\ 
%\cmidrule(l{0em}){1-10} 
 LBB & 3x4x2/3x7x5/3x10x8/3x12x10 & 3/21/171/683 & 48/482/3996/16028
                  & 13/212/3542/22941   \\ \hline
%\cmidrule(l{0em}){1-10} 
 SSHE &  2x2x(1ssh/1oth/2each/2cor)  & 9/21/2648/1201 & 56/135/24116/9406 &14/37/12308/3276  \\ 
%\cmidrule(l{0em}){1-10} 
 SSHB &  2x2x2/2x2x3  & 27/2013 & 318/23643 & 119/13261  \\ \hline
%\cmidrule(l{0em}){1-10} 
 MI &  1x5x(8/10/11)   & 122/753/1506 & 2710/17613/35870 & 1003/11800/34894  \\ 
%\cmidrule(l{0em}){1-10} 
 MIB &  1x5x(8/10/11)   & 138/831/1653 & 3215/20640/41512 & 1668/18591/53349  \\ \hline
% \cmidrule(l{0em}){1-6} 
% Migration(2-2dep) & 1x5x7   & & 237 & 7  & \\ 
%\cmidrule(l{0em}){1-10} 
 LE & 3x3x(2/5)/6x3x2 & 10/46/40 & 178/1269/1239  & 59/467/649 \\
     & 6x3x5/9x2x2 & 132/944  & 5765/12339  & 3798/12230  \\
 \hline

 \end{tabular}
 \caption{Experimental evaluation}
 \label{table:experiments} \vspace{-.5cm}
\end{table}



==> tablelb.tex <==

\begin{wrapfigure}[11]{l}{7.75cm}
	      \vspace{-0.4cm}
 \begin{tabular}{rlrrr}\toprule 
 \multicolumn{1}{c}{\textbf{Name}} &
	      \multicolumn{1}{c}{\textbf{SxHxP}}
 & \multicolumn{1}{c}{\textbf{Execs}} 
 & \multicolumn{1}{c}{\textbf{States}} 
   &\multicolumn{1}{c}{\textbf{Time}}  \\ \toprule  
 
LB & 3x52x50 &  4 & 313 & 1305 \\
LB & 3x102x100 &  4 & 613 & 7301 \\
LB & 3x202x200 &  4 & 1213 & 38203 \\
LB & 3x302x300 &  4 & 1813 & 110220 \\
\hline \hline
LBB & 3x52x50 &  1 & 599 & 11117 \\
LBB & 3x77x75 &  1 & 899 & 31644 \\
LBB & 3x102x100 &  1 & 1199 & 68059 \\
LBB & 3x127x125 &  1 & 1499 & 127740 \\
\hline \hline

\toprule 
 \end{tabular}
\end{wrapfigure}


==> tablele.tex <==

\begin{wrapfigure}[8]{l}{7.35cm}
	      \vspace{-0.45cm}
 \begin{tabular}{rlrrr}\toprule 
 \multicolumn{1}{c}{\textbf{Name}} &
	      \multicolumn{1}{c}{\textbf{SxHxP}}
 & \multicolumn{1}{c}{\textbf{Execs}} 
 & \multicolumn{1}{c}{\textbf{States}} 
   &\multicolumn{1}{c}{\textbf{Time}}  \\ \toprule  
 
LE & 3x3x2 &  3 & 71 & 42 \\
LE & 3x3x5 &  10 & 383 & 355 \\
LE & 6x3x2 &  5 & 217 & 272 \\
LE & 6x3x5 &  16 & 1040 & 2045 \\
LE & 9x2x2 &  10 & 787 & 4570 \\
LE & 15x2x2 &  16 & 2074 & 49274 \\
\hline \hline

\toprule
 \end{tabular}
% \vspace{0.4cm}
%\vspace{2cm}
 \end{wrapfigure}


==> tablemi.tex <==

\begin{wrapfigure}[11]{l}{7.45cm}
	      \vspace{-0.45cm}
 \begin{tabular}{rlrrr}\toprule 
 \multicolumn{1}{c}{\textbf{Name}} &
	      \multicolumn{1}{c}{\textbf{SxHxP}}
 & \multicolumn{1}{c}{\textbf{Execs}} 
 & \multicolumn{1}{c}{\textbf{States}} 
   &\multicolumn{1}{c}{\textbf{Time}}  \\ \toprule  
 
MIb & 1x5x12 &  32 & 599 & 1029 \\
MIb & 1x5x14 &  64 & 1107 & 2730 \\
MIb & 1x5x16 &  748 & 9418 & 24870 \\
MIb & 1x8x20 &  2242 & 45539 & 153419 \\
\hline \hline
MI & 1x5x8 &  32 & 1004 & 865 \\
MI & 1x5x10 &  256 & 9436 & 9176 \\
MI & 1x5x12 &  960 & 17941 & 29675 \\
MI & 1x8x14 &  1727 & 55200 & 119908 \\
\hline \hline

\toprule
 \end{tabular}
 
 \end{wrapfigure}


==> tablessh.tex <==

\begin{wrapfigure}[11]{l}{7.85cm}
	      \vspace{-0.25cm}
 \begin{tabular}{rlrrr}\toprule 
 \multicolumn{1}{c}{\textbf{Name}} &
	      \multicolumn{1}{c}{\textbf{SxHxP}}
 & \multicolumn{1}{c}{\textbf{Execs}} 
 & \multicolumn{1}{c}{\textbf{States}} 
   &\multicolumn{1}{c}{\textbf{Time}}  \\ \toprule  
 
SSH & 2x2x100ssh &  1 & 407 & 83824 \\
SSH & 2x2x120oth &  1 & 490 & 146151 \\
SSH & 2x2x50each &  1 & 410 & 117245 \\
\hline \hline
SSH & 2x2x2cor &  179 & 1691 & 1340 \\
\hline \hline
SSHB & 2x2x2 &  6 & 120 & 104 \\
SSHB & 2x2x3 &  65 & 1419 & 2506 \\
SSHB & 3x3x4 & 421 & 10951 & 33470 \\
\hline \hline
\toprule
%\vspace{-0.2cm}
 \end{tabular}
 
 \end{wrapfigure}

